Dotless Representation of Arabic Text: Analysis and Modeling

This paper presents a novel dotless representation of Arabic text as an alternative to the standard Arabic text representation. We delve into its implications through comprehensive analysis across five diverse corpora and four different tokenization techniques. We explore the impact of dotless representation on the relationships between tokenization granularity and vocabulary size and compare them with standard text representation. Moreover, we analyze the information density of dotless versus standard text using text entropy calculations. To delve deeper into the implications of the dotless representation, statistical and neural language models are constructed using the various text corpora and tokenization techniques. A comparative assessment is then made against language models developed using the standard Arabic text representation. This multifaceted analysis provides valuable insights into the potential advantages and challenges associated with the dotless representation. Last but not the least, utilizing parallel corpora, we draw comparisons between the text analysis of Arabic and English to gain further insights. Our findings shed light on the potential benefits of dotless representation for various NLP tasks, paving the way for further exploration for Arabic natural language processing.

==> tables/lm_datasets_samples_statistics.tex <==
\begin{table}[!ht]
\centering
\begin{tabular}{ccccccc}
\textbf{Dataset}                         & \textbf{samples} & \textbf{N}  & \textbf{V} & \textbf{V`} & \textbf{V/N (\%)} & \textbf{V`/N (\%)} \\ \hline \hline
\multicolumn{1}{c||}{\textbf{quran}}      & 6,057            & 76,911      & 14,748     & 13,229      & 19.175            & 17.2             \\ \hline
\multicolumn{1}{c||}{\textbf{sanadset}}   & 818,354          & 28,759,423  & 317,331    & 227,590     & 1.103             & 0.791              \\ \hline
\multicolumn{1}{c||}{\textbf{poems}}      & 3,090,273        & 29,615,715  & 938,664    & 592,600     & 3.17              & 2.001              \\ \hline
\multicolumn{1}{c||}{\textbf{news}}       & 4,203,375        & 134,427,152 & 892,583    & 654,982     & 0.664             & 0.487              \\ \hline
\multicolumn{1}{c||}{\textbf{wikipedia}}  & 1,440,782        & 62,413,075  & 1,050,038  & 787,643     & 1.682             & 1.262              \\ \hline
\multicolumn{1}{c||}{\textbf{aggregated}} & 9,651,620        & 255,129,750 & 2,067,444  & 1,382,039   & 0.81              & 0.542              \\ \hline
\end{tabular}
\caption{datasets after applying samples selection criteria}
\label{tab:lm_datasets_statistics}
\end{table}

==> tables/tokens_stats_subs.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{@{}cccccccc@{}}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{3}{c}{Subwords (farasa)}            & \multicolumn{3}{c}{Subwords (disjoint)}        \\ \cmidrule(l){3-8} 
\multicolumn{2}{c}{}                         & V         & N                            & H     & V       & N                            & H     \\ \midrule
\multirow{2}{*}{Quran}        & Dotted       & 7,677     & \multirow{2}{*}{129,788}     & 8.240 & 6,484   & \multirow{2}{*}{164,609}     & 7.451 \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-8} 
                              & Dotless      & 6,074     &                              & 7.968 & 4,303   &                              & 6.958 \\ \midrule
\multirow{2}{*}{Sanadset}   & Dotted & 105,469   & \multirow{2}{*}{44,069,593}  & 8.364 & 76,495  & \multirow{2}{*}{55,892,178}  & 7.644 \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-8} 
                              & Dotless      & 74,674    &                              & 8.004 & 37,412  &                              & 7.098 \\ \midrule
\multirow{2}{*}{Ashaar}       & Dotted       & 361,739   & \multirow{2}{*}{57,350,212}  & 9.659 & 191,393 & \multirow{2}{*}{72,437,612}  & 8.480 \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-8} 
                              & Dotless      & 242,735   &                              & 9.148 & 79,968 &                              & 7.687 \\ \midrule
\multirow{2}{*}{Wikipedia}  & Dotted & 1,002,148   & \multirow{2}{*}{303,831,223} & 8.892 & 266,822 & \multirow{2}{*}{412,843,347} & 8.153 \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-8} 
                              & Dotless      & 791,084   &                              & 8.599 & 118,150 &                              & 7.493 \\ \midrule
\multirow{2}{*}{News}         & Dotted       & 344,627   & \multirow{2}{*}{241,222,485} & 8.563 & 151,557 & \multirow{2}{*}{326,024,821} & 7.981 \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-8} 
                              & Dotless      & 263,143   &                              & 8.286 & 68,943  &                              & 7.363 \\ \midrule
\multirow{2}{*}{Aggregated} & Dotted & 1,413,437 & \multirow{2}{*}{646,603,301} & 9.063 & 402,019 & \multirow{2}{*}{867,375,567} & 8.210 \\ \cmidrule(lr){2-3} \cmidrule(lr){5-6} \cmidrule(l){8-8} 
                              & Dotless      & 1,061,481 &                              & 8.711 & 162,389 &                              & 7.523 \\ \bottomrule
\end{tabular}
\caption{Tokens statistics and entropy on subwords tokenizations with datasets from various domains}
\label{tab:tokens_stats_subs}
\end{table}

==> tables/tokens_stats_wc.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{@{}ccccccccc@{}}
\hline
\multicolumn{2}{c}{\multirow{2}{*}{Dataset}} & \multicolumn{4}{c}{Words}                                                 & \multicolumn{3}{c}{Characters}       \\ \cline{3-9} 
\multicolumn{2}{c}{}            & V         & N                        & V/N   & \multicolumn{1}{c|}{H}     & V  & N                        & H    \\ \hline
\multirow{2}{*}{Quran}          & Dotted     & 14,748    & \multirow{2}{*}{77,797}  & 18.96 & \multicolumn{1}{c|}{11.02} & 31 & \multirow{2}{*}{330,709} & 4.15 \\ \cline{2-3} \cline{5-7} \cline{9-9} 
                                & Dotless    & 13,229    &                          & 17    & \multicolumn{1}{c|}{10.87} & 19 &                          & 3.83 \\ \hline
\multirow{2}{*}{Sanadset}       & Dotted     & 317,331   & \multirow{2}{*}{28.88M}  & 1.10  & \multicolumn{1}{c|}{10.92} & 31 & \multirow{2}{*}{112.88M} & 4.24 \\ \cline{2-3} \cline{5-7} \cline{9-9} 
                                & Dotless    & 227,590   &                          & 0.79  & \multicolumn{1}{c|}{10.67} & 19 &                          & 3.86 \\ \hline
\multirow{2}{*}{Ashaar}         & Dotted     & 1,007,279 & \multirow{2}{*}{34.94M}  & 2.88  & \multicolumn{1}{c|}{14.33} & 32 & \multirow{2}{*}{145.57M} & 4.3  \\ \cline{2-3} \cline{5-7} \cline{9-9} 
                                & Dotless    & 631,487   &                          & 1.81  & \multicolumn{1}{c|}{13.70} & 20 &                          & 3.9  \\ \hline
\multirow{2}{*}{Wikipedia}      & Dotted     & 1,811,244 & \multirow{2}{*}{177.42M} & 1.02  & \multicolumn{1}{c|}{13.20} & 31 & \multirow{2}{*}{851.67M} & 4.27 \\ \cline{2-3} \cline{5-7} \cline{9-9} 
                                & Dotless    & 1,345,853 &                          & 0.76   & \multicolumn{1}{c|}{12.94} & 19 &                          & 3.87 \\ \hline
\multirow{2}{*}{News}           & Dotted     & 892,583   & \multirow{2}{*}{134.86M} & 0.66  & \multicolumn{1}{c|}{13.10} & 31 & \multirow{2}{*}{663.80M} & 4.25 \\ \cline{2-3} \cline{5-7} \cline{9-9} 
                                & Dotless    & 654,982   &                          & 0.49  & \multicolumn{1}{c|}{12.87} & 19 &                          & 3.85 \\ \hline
\multirow{2}{*}{Aggregated}     & Dotted     & 2,739,172 & \multirow{2}{*}{376.18M} & 0.73  & \multicolumn{1}{c|}{13.6}  & 31 & \multirow{2}{*}{1.77B}   & 4.27 \\ \cline{2-3} \cline{5-7} \cline{9-9} 
                                & Dotless    & 1,865,126 &                          & 0.50  & \multicolumn{1}{c|}{13.26} & 19 &                          & 3.87 \\ \hline
\end{tabular}
\caption{Tokens statistics and entropy on words and characters tokenizations with datasets from various domains}
\label{tab:tokens_stats_wc}
\end{table}

==> tables/v_ratio_samples_len.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% \begin{table}[]
% \centering
% \begin{tabular}{cccccccc}
% \hline
% \multirow{2}{*}{Dataset} & \multicolumn{2}{c}{Words}                               & \multicolumn{2}{c}{Subwords (farasa)}                   & \multicolumn{2}{c}{Subwords (disjoint)}                 & Characters \\ \cline{2-8} 
%                          & \multicolumn{1}{c|}{V`/V (\%)} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{V`/V (\%)} & \multicolumn{1}{c|}{S} & \multicolumn{1}{c|}{V`/V (\%)} & \multicolumn{1}{c|}{S} & V`/V (\%)  \\ \hline
% Quran                    & \multicolumn{1}{c|}{94.97}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{88.47}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{76.43}     & \multicolumn{1}{c|}{}  & 61.3       \\ \hline
% Sanadset                 & \multicolumn{1}{c|}{80.05}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{79.33}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{62.42}     & \multicolumn{1}{c|}{}  & 61.3       \\ \hline
% Poems                    & \multicolumn{1}{c|}{70.59}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{74.64}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{54.22}     & \multicolumn{1}{c|}{}  & 61.3       \\ \hline
% Wikipedia                & \multicolumn{1}{c|}{81.01}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{84.74}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{58.18}     & \multicolumn{1}{c|}{}  & 61.3       \\ \hline
% News                     & \multicolumn{1}{c|}{81.67}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{83.61}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{61.01}     & \multicolumn{1}{c|}{}  & 61.3       \\ \hline
% Aggregated               & \multicolumn{1}{c|}{75.79}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{81.79}     & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{54.33}     & \multicolumn{1}{c|}{}  & 61.3       \\ \hline
% \end{tabular}
% \caption{Sample lengths and dotless vocabulary ratios}
% \label{tab:v_ratio_samples_len}
% \end{table}



% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\begin{tabular}{cccccccc}
\hline
\multicolumn{2}{c}{Dataset}           & Quran & Sanadset & Ashaar & Wikipedia & News  & Aggregated \\ \hline
\multirow{5}{*}{Words}    & V`/V (\%) & 89.70 & 71.72    & 62.69  & 74.31     & 73.38 & 68.09      \\ \cline{2-8} 
                          & S         & 5.39  & 5.95     & 6.13   & 7.33      & 6.73  & 7.12       \\ \cline{2-8} 
                          & S(10\%)   & 5.06  & 5.31     & 5.37   & 6.41      & 6.14  & 5.91       \\ \cline{2-8} 
                          & S`        & 5.49  & 6.23     & 6.49   & 7.82      & 7.09  & 7.66       \\ \cline{2-8} 
                          & S`(10\%)  & 5.06  & 5.41     & 5.52   & 6.60      & 6.28  & 6.17       \\ \hline
\multirow{5}{*}{farasa}   & V`/V (\%) & 79.12 & 70.80    & 67.10  & 78.94     & 76.36 & 75.10      \\ \cline{2-8} 
                          & S         & 4.46  & 5.50     & 5.79   & 7.32      & 6.45  & 7.14       \\ \cline{2-8} 
                          & S(10\%)   & 3.83  & 4.28     & 4.55   & 5.91      & 5.08  & 5.48       \\ \cline{2-8} 
                          & S`        & 4.65  & 5.89     & 6.22   & 7.81      & 6.88  & 7.66       \\ \cline{2-8} 
                          & S`(10\%)  & 3.86  & 4.42     & 4.81   & 6.36      & 5.39  & 5.87       \\ \hline
\multirow{5}{*}{Disjoint} & V`/V (\%) & 66.36 & 48.91    & 41.78  & 44.28     & 45.49 & 40.39      \\ \cline{2-8} 
                          & S         & 4.06  & 4.95     & 5.16   & 5.54      & 5.31  & 5.59       \\ \cline{2-8} 
                          & S(10\%)   & 3.29  & 4.01     & 4.22   & 4.61      & 4.41  & 4.70       \\ \cline{2-8} 
                          & S`        & 4.29  & 5.31     & 5.56   & 6.07      & 5.75  & 6.11       \\ \cline{2-8} 
                          & S`(10\%)  & 3.41  & 4.14     & 4.39   & 4.87      & 4.60  & 4.89       \\ \hline
Characters                & V`/V (\%) & \multicolumn{6}{c}{61.3}                                   \\ \hline
\end{tabular}
\caption{Sample lengths and dotless vocabulary ratios}
\label{tab:v_ratio_samples_len}
\end{table}
